$C^2M^3$: Cycle-Consistent Multi-Model Merging

In this paper, we present a novel data-free method for merging neural networks in weight space. Differently from most existing works, our method optimizes for the permutations of network neurons globally across all layers. This allows us to enforce cycle consistency of the permutations when merging $N \geq 3$ models, allowing circular compositions of permutations to be computed without accumulating error along the path. We qualitatively and quantitatively motivate the need for such a constraint, showing its benefits when merging sets of models in scenarios spanning varying architectures and datasets. We finally show that, when coupled with activation renormalization, our approach yields the best results in the task.

==> B_experiments/pairwise_barriers_table_cifar100.tex <==
\begin{table}
    \begin{center}
        \begin{tabular}{clccc}
            \toprule
                                                                                                                       & \multirow{2}{*}{\textbf{Matcher}}     & \multicolumn{2}{c}{\textbf{Barrier}}                            \\
                                                                                                                       \cmidrule{3-4}
                                                                                                                       &                      & Train                       & Test            \\
            \midrule
            \parbox[t]{4mm}{\multirow{3}{*}{ \rotatebox[origin=c]{90}{$\underset{8\times}{\text{\texttt{ResNet}}}$} }} & \texttt{Naive}       & 7.00 $\pm$ 1.24                      & 8.37 $\pm$ 1.23          \\
                                                                                                                       & \texttt{Git-Rebasin} & 1.04 $\pm$ 0.10                      & 1.54 $\pm$ 0.13          \\

                                                                                                                       & \texttt{Frank-Wolfe} & $\mathbf{0.92 \pm 0.06}$             & $\mathbf{1.42 \pm 0.10}$ \\
            \midrule
            \parbox[t]{4mm}{\multirow{3}{*}{ \rotatebox[origin=c]{90}{\texttt{VGG16}} }}
                                                                                                                       & \texttt{Naive}       & 5.79 $\pm$ 0.39                      & 7.36 $\pm$ 0.38          \\
                                                                                                                       & \texttt{Git-Rebasin} & 0.44 $\pm$ 0.03                      & 0.64 $\pm$ 0.03          \\
                                                                                                                       & \texttt{Frank-Wolfe} & $\mathbf{0.44 \pm 0.05}$                      & $\mathbf{0.63} \pm 0.06$          \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Mean and standard deviation of the test and train loss barriers for each method when matching $n=2$ models on \texttt{CIFAR100}.}
    \label{tab:pairwise_barriers_table}
\end{table}




==> F_leftovers/content.tex <==
% STUFF THAT DIDN'T MAKE THE CUT FOR NOW

\subsection{Performance matrix of interpolated models} \label{app:performance-matrix}
We report in \cref{fig:perfomance-matrix} the performance of the models interpolated in the universe using the permutations optimized jointly for all $5$ models. It is interesting to note that the performance
\begin{figure}

    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance_orig.pdf}
        \caption{Before mapping to universe.}
        \label{fig:perfomance-matrix-orig}
    \end{subfigure}
    %
    \hfill
    %
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/performance_univ.pdf}
        \caption{After mapping to universe.}
        \label{fig:perfomance-matrix-univ}
    \end{subfigure}

    \caption{Accuracy of the pairwise aggregations of 5 \texttt{ResNet20} trained on \texttt{CIFAR10} with $2\times$ width.}
    \label{fig:perfomance-matrix}
\end{figure}


\begin{table}
    \begin{center}
        \begin{tabular}{lcccc}
            \toprule
            \textbf{Matcher}               & \multicolumn{2}{c}{\textbf{Barrier}}                                 \\
                                           & \textbf{Train}                       & \textbf{Test}                 \\
            \midrule

            \texttt{Naive}                 & 0.098                                & 0.097         & 2.303 & 2.303 \\
            \texttt{Git-Rebasin}           & 0.996                                & 0.983         & 0.013 & 0.067 \\
            \texttt{Git-Rebasin}$^\dagger$ & 0.996                                & 0.983         & 0.013 & 0.067 \\
            \texttt{Frank-Wolfe}           & 0.996                                & 0.983         & 0.013 & 0.066 \\
            \texttt{Frank-Wolfe}$^\dagger$ & 0.996                                & 0.983         & 0.013 & 0.066 \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Mean and standard deviation of the test and train loss barrier for each matcher.}
    \label{tab:MLP_loss_barrier}
\end{table}


